Observation of $\Omega(2012)^- \to \Xi(1530)\bar{K}$ and measurement of the effective couplings of $\Omega(2012)^-$ to $\Xi(1530)\bar{K}$ and $\Xi\bar{K}$

Using $\Upsilon(1S)$, $\Upsilon(2S)$, and $\Upsilon(3S)$ data collected by the Belle detector, we discover a new three-body decay, $\Omega(2012)^-\to\Xi(1530)\bar K\to\Xi\pi\bar K$, with a significance of 5.2~$\sigma$. The mass of the $\Omega(2012)^-$ is $(2012.5\pm0.7\pm0.5)$ MeV and its effective couplings to $\Xi(1530)\bar{K}$ and $\Xi\bar{K}$ are $(39^{+31}_{-39}\pm9)\times10^{-2}$ and $(1.7\pm0.3\pm0.3)\times10^{-2}$, where the first uncertainties are statistical and the second are systematic. The ratio of the branching fraction for the three-body decay to that for the two-body decay to $\Xi\bar{K}$ is $0.99\pm0.26\pm0.06$, assuming isospin symmetry.

==> authors_for_arXiv_submission__one_line_.tex <==
Belle Collaboration: J. K. Ahn, H. Aihara, D. M. Asner, H. Atmacan, R. Ayad, S. Bahinipati, Sw. Banerjee, J. Bennett, M. Bessner, D. Biswas, M. Bra\v{c}ko, P. Branchini, A. Budano, M. Campajola, M.-C. Chang, B. G. Cheon, H. E. Cho, S.-K. Choi, Y. Choi, S. Choudhury, G. De Pietro, R. Dhamija, F. Di Capua, J. Dingfelder, P. Ecker, D. Epifanov, T. Ferber, D. Ferlewicz, B. G. Fulsom, V. Gaur, A. Garmash, A. Giri, P. Goldenzweig, E. Graziani, D. Greenwald, K. Gudkova, C. Hadjivasiliou, D. Herrmann, W.-S. Hou, N. Ipsita, A. Ishikawa, R. Itoh, M. Iwasaki, W. W. Jacobs, S. Jia, Y. Jin, K. K. Joo, C. Kiesling, D. Y. Kim, K.-H. Kim, Y.-K. Kim, K. Kinoshita, P. Kody\v{s}, A. Korobov, E. Kovalenko, P. Kri\v{z}an, P. Krokovny, R. Kumar, K. Kumara, T. Kumita, Y.-J. Kwon, T. Lam, L. K. Li, S. X. Li, Y. B. Li, D. Liventsev, M. Masuda, D. Matvienko, S. K. Maurya, F. Meier, M. Merola, R. Mizuk, R. Mussa, M. Nakao, A. Natochii, M. Niiyama, S. Nishida, P. Pakhlov, G. Pakhlova, S. Pardi, J. Park, T. K. Pedlar, R. Pestotnik, L. E. Piilonen, T. Podobnik, E. Prencipe, M. T. Prim, G. Russo, S. Sandilya, G. Schnell, C. Schwanda, Y. Seino, K. Senyo, W. Shan, C. P. Shen, J.-G. Shiu, A. Sokolov, E. Solovieva, M. Stari\v{c}, M. Sumihama, M. Takizawa, U. Tamponi, K. Tanida, F. Tenchini, Y. Unno, S. Uno, P. Urquijo, Y. Usov, M.-Z. Wang, E. Won, B. D. Yabsley, W. Yan, J. Yelton, J. H. Yin, C. Z. Yuan, L. Yuan, Z. P. Zhang, V. Zhilich, V. Zhukova

==> authors_with_affiliation_s_.tex <==
%%% Paper:    Omega(2012)- to Xi(1530) K-bar
%%% Journal:  Physics Letters B
%%% Contacts: S. Jia, C.P. Shen, C.Z. Yuan
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{pub677} to insert this material into your latex file.
\collab{The Belle Collaboration}
% \author[KEK,SOKENDAI]{I.~Adachi}, % KEK
% \author[LjubljanaJSI]{K.~Adamczyk}, % Ljubljana
  \author[KoreaUnivKU]{J.~K.~Ahn}, % Korea
  \author[UTokyo]{H.~Aihara}, % Tokyo
% \author[Tabuk,KAU]{S.~Al~Said}, % Tabuk
  \author[BNL]{D.~M.~Asner}, % BNL
  \author[Cincinnati]{H.~Atmacan}, % Cincinnati
% \author[BINP,NSU]{V.~Aulchenko}, % BINP
% \author[HSE]{T.~Aushev}, % HSE
  \author[Tabuk]{R.~Ayad}, % Tabuk
% \author[Tata]{T.~Aziz}, % Tata
% \author[IJCLab]{V.~Babu}, % IJCLab
  \author[IITBhubaneswar]{S.~Bahinipati}, % IITB
% \author[Sydney]{A.~M.~Bakich}, % Sydney
% \author[Peking]{Y.~Ban}, % Peking
  \author[Louisville]{Sw.~Banerjee}, % Louisville
% \author[Melbourne]{E.~Barberio}, % Melbourne
% \author[KEK]{M.~Barrett}, % KEK
% \author[Karlsruhe]{M.~Bauer}, % Karlsruhe
% \author[IITMadras]{P.~Behera}, % IITM
% \author[IHEPRussia]{K.~Belous}, % Protvino
  \author[Mississippi]{J.~Bennett}, % Mississippi
% \author[Bonn]{F.~Bernlochner}, % Bonn
  \author[Hawaii]{M.~Bessner}, % Hawaii
% \author[MEPhI]{D.~Besson}, % MEPhI
% \author[IISER]{V.~Bhardwaj}, % IISERM
% \author[IITGuwahati]{B.~Bhuyan}, % IITG
% \author[DESY]{T.~Bilka}, % DESY
% \author[LMU]{S.~Bilokin}, % LMU
  \author[Louisville]{D.~Biswas}, % Louisville
% \author[KEK]{T.~Bloomfield}, % KEK
% \author[BINP,NSU]{A.~Bobrov}, % BINP
% \author[HSE,Soochow]{D.~Bodrov}, % HSE
% \author[BINP,NSU]{A.~Bondar}, % BINP
% \author[WayneState]{G.~Bonvicini}, % WayneState
% \author[LjubljanaJSI]{J.~Borah}, % Ljubljana
% \author[Krakow]{A.~Bozek}, % Krakow
  \author[LjubljanaUM,LjubljanaJSI]{M.~Bra\v{c}ko}, % Ljubljana
  \author[RomaTreINFN]{P.~Branchini}, % RomaTre
% \author[Hawaii]{T.~E.~Browder}, % Hawaii
  \author[RomaTreINFN]{A.~Budano}, % RomaTre
  \author[NapoliINFN,NapoliUNIV]{M.~Campajola}, % Napoli
% \author[DESY]{L.~Cao}, % DESY
% \author[Prague]{D.~\v{C}ervenkov}, % Charles
  \author[FuJen]{M.-C.~Chang}, % FuJen
% \author[NTUTaiwan]{P.~Chang}, % Taiwan
% \author[MPP]{V.~Chekelian}, % MPI
% \author[NCU]{A.~Chen}, % NCU
% \author[ISU]{C.~Chen}, % ISU
% \author[USTC]{Y.~Chen}, % USTC
% \author[NTUTaiwan]{Y.-T.~Chen}, % Taiwan
  \author[Hanyang]{B.~G.~Cheon}, % Hanyang
% \author[BINP]{K.~Chilikin}, % BINP
  \author[Hanyang]{H.~E.~Cho}, % Hanyang
% \author[KISTI]{K.~Cho}, % KISTI
% \author[Yonsei]{S.-J.~Cho}, % Yonsei
  \author[CAU]{S.-K.~Choi}, % CAU
  \author[SKKU]{Y.~Choi}, % Sungkyunkwan
  \author[ISU]{S.~Choudhury}, % ISU
% \author[ISU]{J.~Cochran}, % ISU
% \author[DESY]{S.~Cunliffe}, % DESY
% \author[IPMU]{T.~Czank}, % IPMU
% \author[MNITJaipur]{S.~Das}, % MNIT
% \author[IITMadras]{N.~Dash}, % IITM
% \author[LjubljanaJSI]{G.~de~Marino}, % Ljubljana
% \author[NapoliINFN,NapoliUNIV]{G.~De~Nardo}, % Napoli
  \author[Karlsruhe]{G.~De~Pietro}, % Karlsruhe
  \author[IITHyderabad]{R.~Dhamija}, % IITH
  \author[NapoliINFN,NapoliUNIV]{F.~Di~Capua}, % Napoli
  \author[Bonn]{J.~Dingfelder}, % Bonn
% \author[Prague]{Z.~Dole\v{z}al}, % Charles
% \author[ITAR]{T.~V.~Dong}, % DuyTan
% \author[Melbourne]{D.~Dossett}, % Melbourne
% \author[Hawaii]{S.~Dubey}, % Hawaii
  \author[Karlsruhe]{P.~Ecker}, % Karlsruhe
  \author[BINP,NSU]{D.~Epifanov}, % BINP
% \author[Karlsruhe]{M.~Feindt}, % Karlsruhe
  \author[Karlsruhe]{T.~Ferber}, % Karlsruhe
  \author[Melbourne]{D.~Ferlewicz}, % Melbourne
% \author[Goettingen]{A.~Frey}, % Goettingen
  \author[PNNL]{B.~G.~Fulsom}, % PNNL
% \author[BINP,NSU]{N.~Gabyshev}, % BINP
% \author[CMU]{R.~Garg}, % CMU
  \author[UPES]{V.~Gaur}, % UPES
  \author[BINP,NSU]{A.~Garmash}, % BINP
  \author[IITHyderabad]{A.~Giri}, % IITH
  \author[Karlsruhe]{P.~Goldenzweig}, % Karlsruhe
% \author[LjubljanaUniLJ,NovaGorica,LjubljanaJSI]{B.~Golob}, % Ljubljana
% \author[USTC]{G.~Gong}, % USTC
  \author[RomaTreINFN]{E.~Graziani}, % RomaTre
  \author[TUM]{D.~Greenwald}, % TUM
% \author[Pittsburgh]{T.~Gu}, % Pittsburgh
% \author[Cincinnati]{Y.~Guan}, % Cincinnati
  \author[BINP,NSU]{K.~Gudkova}, % BINP
  \author[PNNL]{C.~Hadjivasiliou}, % PNNL
% \author[HEPHYVienna]{H.~Haigh}, % Vienna
% \author[Tata]{S.~Halder}, % Tata
% \author[Beihang]{X.~Han}, % Beihang
% \author[KEK,SOKENDAI]{K.~Hara}, % KEK
% \author[KEK,SOKENDAI]{T.~Hara}, % KEK
% \author[Hawaii]{O.~Hartbrich}, % Hawaii
% \author[Niigata]{K.~Hayasaka}, % Niigata
% \author[NaraWu]{H.~Hayashii}, % Nara
% \author[MPP]{S.~Hazra}, % MPI
% \author[Bonn]{M.~T.~Hedges}, % Bonn
  \author[WayneState]{D.~Herrmann}, % WayneState
% \author[BNL,DESY]{M.~Hern\'{a}ndez~Villanueva}, % BNL
% \author[IPMU]{T.~Higuchi}, % IPMU
% \author[Nagoya]{H.~Hirata}, % Nagoya
  \author[NTUTaiwan]{W.-S.~Hou}, % Taiwan
% \author[Sydney]{C.-L.~Hsu}, % Sydney
% \author[NTUTaiwan]{K.~Huang}, % Taiwan
% \author[NagoyaKMI,Nagoya]{T.~Iijima}, % Nagoya
% \author[Nagoya,KEK]{K.~Inami}, % Nagoya
% \author[HEPHYVienna]{G.~Inguglia}, % Vienna
  \author[IITHyderabad]{N.~Ipsita}, % IITH
  \author[KEK,SOKENDAI]{A.~Ishikawa}, % KEK
  \author[KEK,SOKENDAI]{R.~Itoh}, % KEK
  \author[OsakaMetropolitan]{M.~Iwasaki}, % OsakaCity
% \author[KEK]{Y.~Iwasaki}, % KEK
% \author[TokyoMetropolitan]{S.~Iwata}, % TMU
  \author[Indiana]{W.~W.~Jacobs}, % Indiana
% \author[Gyeongsang]{E.-J.~Jang}, % Gyeongsang
% \author[Kyungpook]{H.~B.~Jeon}, % Kyungpook
% \author[HNU]{Q.~P.~Ji}, % HNU
  \author[SEU]{S.~Jia}, % SEU
  \author[BNL]{Y.~Jin}, % BNL
  \author[Chonnam]{K.~K.~Joo}, % Chonnam
% \author[TokyoMetropolitan]{H.~Kakuno}, % TMU
% \author[IITGuwahati]{D.~Kalita}, % IITG
% \author[HEPHYVienna]{A.~B.~Kaliyar}, % Vienna
% \author[IPMU]{K.~H.~Kang}, % IPMU
% \author[ISU]{S.~Kang}, % ISU
% \author[Krakow]{P.~Kapusta}, % Krakow
% \author[DESY]{G.~Karyan}, % DESY
% \author[Chiba]{H.~Kawai}, % Chiba
% \author[Kitasato]{T.~Kawasaki}, % Kitasato
% \author[KEK]{H.~Kichimi}, % KEK
  \author[MPP]{C.~Kiesling}, % MPI
% \author[Hanyang]{C.~H.~Kim}, % Hanyang
  \author[Soongsil]{D.~Y.~Kim}, % Soongsil
% \author[Kyungpook]{H.~J.~Kim}, % Kyungpook
  \author[KISTI]{K.-H.~Kim}, % KISTI
% \author[Seoul]{S.~K.~Kim}, % Seoul
% \author[KoreaUnivKU]{Y.~J.~Kim}, % Korea
  \author[Yonsei]{Y.-K.~Kim}, % Yonsei
% \author[VPI]{T.~D.~Kimmel}, % VPI
% \author[VPI,KEK]{H.~Kindo}, % VPI
  \author[Cincinnati]{K.~Kinoshita}, % Cincinnati
% \author[DESY]{C.~Kleinwort}, % DESY
  \author[Prague]{P.~Kody\v{s}}, % Charles
% \author[DESY]{I.~Komarov}, % DESY
% \author[Kitasato]{T.~Konno}, % Kitasato
  \author[BINP,NSU]{A.~Korobov}, % BINP
% \author[LjubljanaUM,LjubljanaJSI]{S.~Korpar}, % Ljubljana
% \author[IJCLab]{E.~Kou}, % IJCLab
  \author[BINP,NSU]{E.~Kovalenko}, % BINP
  \author[LjubljanaUniLJ,LjubljanaJSI]{P.~Kri\v{z}an}, % Ljubljana
% \author[Mississippi]{R.~Kroeger}, % Mississippi
% \author[Melbourne]{J.-F.~Krohn}, % Melbourne
  \author[BINP,NSU]{P.~Krokovny}, % BINP
% \author[LMU]{T.~Kuhr}, % LMU
% \author[IITGuwahati]{D.~Kumar}, % IITG
% \author[IISER]{M.~Kumar}, % IISERM
  \author[PanjabPAU]{R.~Kumar}, % Punjab
  \author[Mississippi]{K.~Kumara}, % Mississippi
  \author[TokyoMetropolitan]{T.~Kumita}, % TMU
% \author[Chiba]{E.~Kurihara}, % Chiba
% \author[BINP,NSU]{A.~Kuzmin}, % BINP
% \author[Prague]{P.~Kvasni\v{c}ka}, % Charles
  \author[Yonsei]{Y.-J.~Kwon}, % Yonsei
% \author[KEK]{Y.-T.~Lai}, % KEK
% \author[MNITJaipur]{K.~Lalwani}, % MNIT
  \author[VPI]{T.~Lam}, % VPI
% \author[Giessen]{J.~S.~Lange}, % Giessen
% \author[Hanyang]{I.~S.~Lee}, % Hanyang
% \author[Seoul]{J.~K.~Lee}, % Seoul
% \author[Kyungpook]{S.~C.~Lee}, % Kyungpook
% \author[KEK]{D.~Levit}, % KEK
% \author[Hawaii]{P.~Lewis}, % Hawaii
% \author[LNNU]{C.~H.~Li}, % LNNU
  \author[Cincinnati]{L.~K.~Li}, % Cincinnati
  \author[Fudan]{S.~X.~Li}, % Fudan
% \author[Fudan]{Y.~Li}, % Fudan
  \author[Fudan]{Y.~B.~Li}, % Fudan
% \author[MPP]{L.~Li~Gioi}, % MPI
% \author[IITMadras]{J.~Libby}, % IITM
% \author[NTUTaiwan]{Y.-R.~Lin}, % Taiwan
% \author[Hiroshima]{Z.~Liptak}, % Hiroshima
  \author[WayneState,KEK]{D.~Liventsev}, % WayneState
% \author[Fudan]{T.~Luo}, % Fudan
% \author[RIKENMSL]{Y.~Ma}, % NPC
% \author[UOM]{J.~MacNaughton}, % NPC
% \author[IITBhubaneswar]{S.~Maity}, % IITB
% \author[DESY]{A.~Martini}, % DESY
  \author[Eri,RCNP]{M.~Masuda}, % NPC
% \author[UOM]{T.~Matsuda}, % NPC
  \author[BINP,NSU]{D.~Matvienko}, % BINP
  \author[IITGuwahati]{S.~K.~Maurya}, % IITG
  \author[Duke]{F.~Meier}, % Duke
  \author[NapoliINFN,NapoliUNIV]{M.~Merola}, % Napoli
% \author[Bonn]{F.~Metzner}, % Bonn
% \author[NaraWu,KEK]{K.~Miyabayashi}, % Nara
% \author[KEK,SOKENDAI]{H.~Miyake}, % KEK
% \author[Niigata]{H.~Miyata}, % Niigata
  \author[IJCLab]{R.~Mizuk}, % IJCLab
% \author[Tata]{G.~B.~Mohanty}, % Tata
% \author[KoreaUnivKU]{H.~K.~Moon}, % Korea
% \author[Seoul]{T.~J.~Moon}, % Seoul
% \author[MPP]{H.-G.~Moser}, % MPI
% \author[HEPHYVienna]{M.~Mrvar}, % Vienna
% \author[Karlsruhe]{T.~M\"uller}, % Karlsruhe
  \author[TorinoINFN]{R.~Mussa}, % Torino
% \author[KEK,SOKENDAI]{I.~Nakamura}, % KEK
% \author[KEK,SOKENDAI]{K.~R.~Nakamura}, % KEK
% \author[OsakaMetropolitan]{E.~Nakano}, % OsakaCity
% \author[RCNP]{T.~Nakano}, % NPC
  \author[KEK,SOKENDAI]{M.~Nakao}, % KEK
% \author[KEK,SOKENDAI]{H.~Nakayama}, % KEK
% \author[NTUTaiwan]{H.~Nakazawa}, % Taiwan
% \author[Krakow]{Z.~Natkaniec}, % Krakow
  \author[Hawaii]{A.~Natochii}, % Hawaii
% \author[IITHyderabad]{L.~Nayak}, % IITH
% \author[TelAviv]{M.~Nayak}, % TelAviv
% \author[DESY]{C.~Niebuhr}, % DESY
  \author[KSU]{M.~Niiyama}, % NPC
% \author[BNL]{N.~K.~Nisar}, % BNL
  \author[KEK,SOKENDAI,Niigata]{S.~Nishida}, % KEK
% \author[Hawaii]{K.~Nishimura}, % Hawaii
% \author[Niigata]{K.~Ogawa}, % Niigata
% \author[Toho]{S.~Ogawa}, % Toho
% \author[Kanagawa]{S.~Okuno}, % Kanagawa
% \author[CAU]{S.~L.~Olsen}, % CAU
% \author[NDU,Niigata]{H.~Ono}, % NihonDental
% \author[UTokyo]{Y.~Onuki}, % Tokyo
% \author[IJCLab]{P.~Oskin}, % IJCLab
% \author[KEK,SOKENDAI]{H.~Ozaki}, % KEK
  \author[HSE]{P.~Pakhlov}, % HSE
  \author[HSE]{G.~Pakhlova}, % HSE
  \author[NapoliINFN]{S.~Pardi}, % Napoli
% \author[Kyungpook]{H.~Park}, % Kyungpook
  \author[Yonsei]{J.~Park}, % Yonsei
% \author[KEK]{S.-H.~Park}, % KEK
% \author[RomaTreINFN]{A.~Passeri}, % RomaTre
% \author[Louisville]{S.~Patra}, % Louisville
% \author[TUM]{S.~Paul}, % TUM
  \author[Luther]{T.~K.~Pedlar}, % Luther
  \author[LjubljanaJSI]{R.~Pestotnik}, % Ljubljana
% \author[Melbourne]{F.~Pham}, % Melbourne
  \author[VPI]{L.~E.~Piilonen}, % VPI
  \author[LjubljanaUniLJ,LjubljanaJSI]{T.~Podobnik}, % Ljubljana
% \author[TelAviv,HSE]{V.~Popov}, % TelAviv
% \author[ISU]{S.~Prell}, % ISU
  \author[Giessen]{E.~Prencipe}, % Giessen
  \author[Bonn]{M.~T.~Prim}, % Bonn
% \author[SouthCarolina]{M.~V.~Purohit}, % SouthCarolina
% \author[TUM]{A.~Rabusov}, % TUM
% \author[LMU]{M.~Ritter}, % LMU
% \author[DESY]{M.~R\"{o}hrken}, % DESY
% \author[DESY]{A.~Rostomyan}, % DESY
% \author[TriesteINFN]{N.~Rout}, % Trieste
% \author[Krakow]{M.~Rozanska}, % Krakow
  \author[NapoliUNIV]{G.~Russo}, % Napoli
% \author[ISU]{D.~Sahoo}, % ISU
% \author[KEK,SOKENDAI]{Y.~Sakai}, % KEK
% \author[Malaya,LMU]{M.~Salehi}, % Malaya
  \author[IITHyderabad]{S.~Sandilya}, % IITH
% \author[Cincinnati]{A.~Sangal}, % Cincinnati
% \author[LjubljanaUniLJ,LjubljanaJSI]{L.~Santelj}, % Ljubljana
% \author[Tohoku]{T.~Sanuki}, % Tohoku
% \author[KEK]{Y.~Sato}, % KEK
% \author[Pittsburgh]{V.~Savinov}, % Pittsburgh
% \author[LMU]{P.~Schmolz}, % LMU
% \author[EPFL]{O.~Schneider}, % Lausanne
  \author[Bilbao,IKERBASQUE]{G.~Schnell}, % Bilbao
% \author[Hawaii]{J.~Schueler}, % Hawaii
  \author[HEPHYVienna]{C.~Schwanda}, % Vienna
% \author[Cincinnati]{A.~J.~Schwartz}, % Cincinnati
% \author[Goettingen]{B.~Schwenker}, % Goettingen
% \author[RIKENBNL]{R.~Seidl}, % RIKEN
  \author[Niigata]{Y.~Seino}, % Niigata
  \author[Yamagata]{K.~Senyo}, % Yamagata
% \author[Melbourne]{M.~E.~Sevior}, % Melbourne
  \author[HUNNU]{W.~Shan}, % HUNNU
% \author[IHEPRussia]{M.~Shapkin}, % Protvino
% \author[MNITJaipur]{C.~Sharma}, % MNIT
% \author[Hawaii]{V.~Shebalin}, % Hawaii
  \author[Fudan]{C.~P.~Shen}, % Fudan
% \author[Toho]{H.~Shibuya}, % Toho
  \author[NTUTaiwan]{J.-G.~Shiu}, % Taiwan
% \author[BINP,NSU]{B.~Shwartz}, % BINP
% \author[Hawaii]{A.~Sibidanov}, % Hawaii
% \author[Karlsruhe]{F.~Simon}, % Karlsruhe
% \author[Panjab,UPES]{J.~B.~Singh}, % Panjab
% \author[Chennai]{R.~Sinha}, % IMSC
% \author[Melbourne]{K.~Smith}, % Melbourne
  \author[IHEPRussia]{A.~Sokolov}, % Protvino
% \author[DESY]{Y.~Soloviev}, % DESY
  \author[BINP]{E.~Solovieva}, % BINP
% \author[NovaGorica]{S.~Stani\v{c}}, % NovaGorica
  \author[LjubljanaJSI]{M.~Stari\v{c}}, % Ljubljana
% \author[VPI]{Z.~S.~Stottler}, % VPI
% \author[PNNL]{J.~F.~Strube}, % PNNL
% \author[Krakow]{J.~Stypula}, % Krakow
  \author[Gifu,RCNP]{M.~Sumihama}, % NPC
% \author[KEK,SOKENDAI,NaraWu]{K.~Sumisawa}, % KEK
% \author[TokyoMetropolitan]{T.~Sumiyoshi}, % TMU
% \author[Bonn]{W.~Sutcliffe}, % Bonn
% \author[KEK,SOKENDAI]{S.~Y.~Suzuki}, % KEK
  \author[SPU,JPARC,RIKENMSL]{M.~Takizawa}, % NPC
  \author[TorinoINFN]{U.~Tamponi}, % Torino
% \author[KEK,SOKENDAI]{S.~Tanaka}, % KEK
% \author[Fudan]{S.~S.~Tang}, % Fudan
  \author[JAEA]{K.~Tanida}, % NPC
% \author[KEK]{N.~Taniguchi}, % KEK
% \author[Florida]{Y.~Tao}, % Florida
% \author[Melbourne]{G.~N.~Taylor}, % Melbourne
  \author[PisaINFN,PisaUNIV]{F.~Tenchini}, % Pisa
% \author[OsakaMetropolitan]{Y.~Teramoto}, % OsakaCity
% \author[Tata]{R.~Tiwary}, % Tata
% \author[IJCLab]{K.~Trabelsi}, % IJCLab
% \author[KEK,SOKENDAI]{T.~Tsuboyama}, % KEK
% \author[Nagoya]{N.~Tsuzuki}, % Nagoya
% \author[Titech]{M.~Uchida}, % NPC
% \author[KEK,SOKENDAI]{I.~Ueda}, % KEK
% \author[KEK,SOKENDAI]{S.~Uehara}, % KEK
% \author[HSE]{T.~Uglov}, % HSE
  \author[Hanyang]{Y.~Unno}, % Hanyang
% \author[KEK]{K.~Uno}, % KEK
  \author[KEK,SOKENDAI]{S.~Uno}, % KEK
  \author[Melbourne]{P.~Urquijo}, % Melbourne
% \author[KEK,UTokyo,SOKENDAI]{Y.~Ushiroda}, % KEK
  \author[BINP,NSU]{Y.~Usov}, % BINP
% \author[Hawaii]{S.~E.~Vahsen}, % Hawaii
% \author[Hawaii]{G.~Varner}, % Hawaii
% \author[Sydney]{K.~E.~Varvell}, % Sydney
% \author[BINP,NSU]{A.~Vinokurova}, % BINP
% \author[Duke]{A.~Vossen}, % Duke
% \author[KEK]{E.~Waheed}, % KEK
% \author[MPP]{B.~Wang}, % MPI
% \author[NUUTaiwan]{C.~H.~Wang}, % NUU
% \author[Florida]{D.~Wang}, % Florida
% \author[Pittsburgh]{E.~Wang}, % Pittsburgh
  \author[NTUTaiwan]{M.-Z.~Wang}, % Taiwan
% \author[Fudan]{X.~L.~Wang}, % Fudan
% \author[Niigata]{M.~Watanabe}, % Niigata
% \author[Kanagawa]{Y.~Watanabe}, % Kanagawa
% \author[Cincinnati]{S.~Watanuki}, % Cincinnati
% \author[DESY]{S.~Wehle}, % DESY
% \author[TriesteINFN]{O.~Werbycka}, % Trieste
% \author[SMI]{E.~Widmann}, % Vienna
% \author[Krakow]{J.~Wiechczynski}, % Krakow
  \author[KoreaUnivKU]{E.~Won}, % Korea
% \author[Soochow]{X.~Xu}, % Soochow
  \author[Sydney]{B.~D.~Yabsley}, % Sydney
% \author[KEK]{S.~Yamada}, % KEK
% \author[Tohoku]{H.~Yamamoto}, % Tohoku
  \author[USTC]{W.~Yan}, % USTC
% \author[KoreaUnivKU]{S.~B.~Yang}, % Korea
% \author[DESY]{H.~Ye}, % DESY
  \author[Florida]{J.~Yelton}, % Florida
  \author[KoreaUnivKU]{J.~H.~Yin}, % Korea
% \author[IHEPChina]{Y.~Yook}, % IHEP
  \author[IHEPChina]{C.~Z.~Yuan}, % IHEP
  \author[Beihang]{L.~Yuan}, % Beihang
% \author[Niigata]{Y.~Yusa}, % Niigata
% \author[ISU]{Y.~Zhai}, % ISU
% \author[IHEPChina]{J.~Zhang}, % IHEP
  \author[USTC]{Z.~P.~Zhang}, % USTC
  \author[BINP,NSU]{V.~Zhilich}, % BINP
  \author[LjubljanaUniLJ,LjubljanaJSI]{V.~Zhukova}, % Ljubljana
% \author[BINP,NSU]{V.~Zhulanov} % BINP
%%%\address[Goettingen]{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\address[Beihang]{Beihang University, Beijing 100191, China}
\address[BNL]{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\address[BINP]{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
%%%\address[CMU]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\address[Prague]{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
%%%\address[Chiba]{Chiba University, Chiba 263-8522, Japan}
\address[Chonnam]{Chonnam National University, Gwangju 61186, South Korea}
\address[CAU]{Chung-Ang University, Seoul 06974, South Korea}
%%%\address[DESY]{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\address[Duke]{Duke University, Durham, North Carolina 27708, U.S.A.}
%%%\address[ITAR]{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
%%%\address[EPFL]{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015, Switzerland}
\address[FuJen]{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\address[Fudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\address[Gifu]{Gifu University, Gifu 501-1193, Japan}
\address[SOKENDAI]{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
%%%\address[Gyeongsang]{Gyeongsang National University, Jinju 52828, South Korea}
\address[Hanyang]{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
%%%\address[HNU]{Henan Normal University, Xinxiang 453007, China}
\address[KEK]{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\address[JPARC]{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
%%%\address[Hiroshima]{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\address[HUNNU]{Hunan Normal University, Changsha 410081, China}
\address[IKERBASQUE]{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao, Spain}
\address[NapoliINFN]{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\address[PisaINFN]{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\address[RomaTreINFN]{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\address[TorinoINFN]{INFN Sezione di Torino, I-10125 Torino, Italy}
%%%\address[TriesteINFN]{INFN Sezione di Trieste, I-34127 Trieste, Italy}
%%%\address[IISER]{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\address[IITBhubaneswar]{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\address[IITGuwahati]{Indian Institute of Technology Guwahati, Assam 781039, India}
\address[IITHyderabad]{Indian Institute of Technology Hyderabad, Telangana 502285, India}
%%%\address[IITMadras]{Indian Institute of Technology Madras, Chennai 600036, India}
\address[Indiana]{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\address[IHEPRussia]{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\address[HEPHYVienna]{Institute of High Energy Physics, Vienna 1050, Austria}
\address[IHEPChina]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
%%%\address[Chennai]{Institute of Mathematical Sciences, Chennai 600113, India}
\address[ISU]{Iowa State University, Ames, Iowa 50011, U.S.A.}
\address[JAEA]{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
%%%\address[Kanagawa]{Kanagawa University, Yokohama 221-8686, Japan}
\address[Karlsruhe]{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
%%%\address[KAU]{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589, Saudi Arabia}
%%%\address[Kitasato]{Kitasato University, Sagamihara 252-0373, Japan}
\address[KISTI]{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\address[KoreaUnivKU]{Korea University, Seoul 02841, South Korea}
\address[KSU]{Kyoto Sangyo University, Kyoto 603-8555, Japan}
%%%\address[Kyungpook]{Kyungpook National University, Daegu 41566, South Korea}
%%%\address[LNNU]{Liaoning Normal University, Dalian 116029, China}
\address[Giessen]{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\address[Luther]{Luther College, Decorah, Iowa 52101, U.S.A.}
%%%\address[MNITJaipur]{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
%%%\address[LMU]{Ludwig Maximilians University, 80539 Munich, Germany}
%%%\address[SMI]{Stefan Meyer Institute for Subatomic Physics, Vienna 1090, Austria}
%%%\address[MEPhI]{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
%%%\address[Nagoya]{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
%%%\address[NagoyaKMI]{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
%%%\address[NaraWu]{Nara Women's University, Nara 630-8506, Japan}
%%%\address[NCU]{National Central University, Chung-li 32054, Taiwan}
\address[HSE]{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\address[NTUTaiwan]{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
%%%\address[NUUTaiwan]{National United University, Miao Li 36003, Taiwan}
%%%\address[Krakow]{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\address[Niigata]{Niigata University, Niigata 950-2181, Japan}
%%%\address[NDU]{Nippon Dental University, Niigata 951-8580, Japan}
\address[NSU]{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\address[OsakaMetropolitan]{Osaka Metropolitan University, Osaka 558-8585, Japan}
\address[RCNP]{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\address[PNNL]{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
%%%\address[Panjab]{Panjab University, Chandigarh 160014, India}
%%%\address[Peking]{Peking University, Beijing 100871, China}
\address[MPP]{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\address[PanjabPAU]{Punjab Agricultural University, Ludhiana 141004, India}
\address[RIKENMSL]{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\address[RIKENBNL]{RIKEN BNL Research Center, Upton, New York 11973, U.S.A.}
%%%\address[Seoul]{Seoul National University, Seoul 08826, South Korea}
\address[SPU]{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
%%%\address[Soochow]{Soochow University, Suzhou 215006, China}
\address[Soongsil]{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
%%%\address[SouthCarolina]{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\address[SEU]{Southeast University, Nanjing 211189, China}
\address[LjubljanaJSI]{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\address[SKKU]{Sungkyunkwan University, Suwon 16419, South Korea}
%%%\address[Tata]{Tata Institute of Fundamental Research, Mumbai 400005, India}
\address[TUM]{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
%%%\address[TelAviv]{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
%%%\address[Toho]{Toho University, Funabashi 274-8510, Japan}
%%%\address[Tohoku]{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
%%%\address[Titech]{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\address[TokyoMetropolitan]{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\address[NapoliUNIV]{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\address[PisaUNIV]{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
%%%\address[RomaTreUNIV]{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\address[IJCLab]{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\address[Bilbao]{Department of Physics \& EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao, Spain}
\address[Bonn]{University of Bonn, 53115 Bonn, Germany}
\address[Cincinnati]{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\address[Florida]{University of Florida, Gainesville, Florida 32611, U.S.A.}
\address[Hawaii]{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\address[LjubljanaUniLJ]{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\address[Louisville]{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
%%%\address[Malaya]{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
%%%\address[LjubljanaUM]{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\address[Melbourne]{School of Physics, University of Melbourne, Victoria 3010, Australia}
\address[Mississippi]{University of Mississippi, University, Mississippi 38677, U.S.A.}
%%%\address[UOM]{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\address[NovaGorica]{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\address[UPES]{University of Petroleum and Energy Studies, Dehradun 248007, India}
%%%\address[Pittsburgh]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\address[USTC]{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\address[Sydney]{School of Physics, University of Sydney, New South Wales 2006, Australia}
\address[Tabuk]{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\address[UTokyo]{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\address[Eri]{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
%%%\address[IPMU]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
%%%\address[Utkal]{Utkal University, Bhubaneswar 751004, India}
\address[VPI]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\address[WayneState]{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\address[Yamagata]{Yamagata University, Yamagata 990-8560, Japan}
\address[Yonsei]{Yonsei University, Seoul 03722, South Korea}
